AppWorld-UL: Benchmarking Diverse Agent-User Interactions for Tool-Use

Tool-use agents that address day-to-day digital tasks such as ordering groceries must not only operate applications, but also interact with the user, e.g., to ask clarification questions, prompt for confirmation, and inform the user when the instruction is infeasible. However, current benchmarks for evaluating agent-user interactions do not capture the diversity of such interactions. Further, they operate in small environments with few, often non-state-changing, APIs. To address this gap, we introduce AppWorld-UL, a ``user-in-the-loop'' benchmark of 516 challenging tasks requiring diverse agent-user interactions. Building upon the AppWorld framework with 9 popular simulated apps like Amazon and Spotify, we systematically modify original tasks to introduce ambiguities and constraints that necessitate various types of agent-user interaction. User behavior is simulated by an LLM prompted to respond with carefully designed knowledge boundaries, offering more reliable simulation than the unconstrained or overly rigid alternatives used in prior work. Our evaluation reveals that a state-of-the-art LLM, Claude Opus 4.7, achieves only 48.6% success on AppWorld-UL, and only 35.7% on the harder, compositional subset. On the stricter, scenario-level metric, compositional task performance drops to only 21.3%. Our analysis reveals that correct user-interaction is crucial for success. This demonstrates the benchmark's difficulty and its potential to advance research on user-in-the-loop tool-use agents.

==> _sections/introduction-scratch.tex <==
\section{Introduction}
\ashish{test}
\niranjan{test}
\tejas{test}
\michael{test}
\harsh{test}
\junzhi{test}
\jane{test}

%\jane{
% 1. LLM-based agents are pretty good, even when evaluated on more realistic tasks.
% 2. But in reality, XYZ cases happen as a result of user-model interaction dynamics. (cite more HCI-coded studies)
% 3. We find that in simulated task settings with ABC interaction modes, DEF types of failures surface from model interactions with users]
% 4. Current benchmarks fail to model these XYZ cases. So we introduce a benchmark that does.
% 5. (Brief summary of benchmark)
% 6. Overall, ...(conclusion)
% }

\ashish{General note: As Jane mentions in several places, the intro feels a bit too tied to AppWorld. I see two paths: (A) double-down on the AppWorld ``extension'' route, in which case the key points to highlight would be what AppWorld is missing and how this extension fixes that. In other words, after the broad motivation (first two paragraphs), go specifically into pointing out the \emph{shortcomings} (not strengths!) of AppWorld, and then say how this extension fixes it.  (B) Alternatively, pitch this as a way of creating agent-user interactive tasks that's superior to the ways that exist. In this case, after the broad motivation, state why this proposed way of injecting interaction is better than what exists (in a general way), what are the rich types of interactions proposed, why are these realistic/reasonable, etc.; then say we start with AppWorld as the base / backbone because of a, b, c (just briefly). In this approach, AppWorld's strength are inherited and mentioned, but it would still take a sort of back seat.}

\ashish{give the above some thought and let's discuss when we meet!} \harsh{I am leaning towards (B).}

Agents based on large language models (LLMs) have demonstrated remarkable capabilities across various domains, including reasoning, code generation, and complex applications such as video games and web search. In the real world, the task solving process of agent is highly collaborative, where human users often begin with only a vague or partially formed intent, and iteratively refine or augment their goals as the agent explores the environment and provides new information.

However, most existing agent benchmarks offer only clear, solvable, and fully specified tasks environment, leaving the user–agent interaction dimension unaddressed. As a result, although many agent systems show strong performance on these controlled benchmarks, they frequently fail in real-world scenarios: they may hallucinate missing details instead of requesting clarification, misinterpret ambiguous instructions, proceed with potentially unsafe actions without seeking user confirmation, or fail to adapt their plans when users revise or refine their goals. 
\jane{Cite recent ($\geq$ 2025) studies that demonstrate this is the case with user studies.}

\begin{figure*}[htb]
    \centering
    \scalebox{0.99}{
    \includegraphics[width=1\linewidth]{figures/example_solving_process.pdf}
    }
    \caption{example}
    \label{fig:example_solving_process}
\end{figure*}

In recent years, several works have begun to incorporate the agent–user interaction dimension into their benchmarks, marking an important step toward evaluating collaborative agent capabilities. However, these benchmarks remain limited in several key aspects: 
\jane{All of these benchmarks need citations.}
(1) Many rely on LLM-generated tasks, which often lack consistency, controllability, and grounding in realistic user needs. 
\jane{I'm personally not sure if we should lead with this. I feel that some well-regarded benchmarks are partially LLM-generated and I don't think it's the strongest thing we bring to the table.}
\ashish{different point: if our ``solution'' to this issue is to simply start with AppWorld and benefit from its realism, this isn't the strongest point to lead with. However, if the intent here is to highlight ``manual perturbations'', then maybe this can work, but then it needs to be worded appropriately.}
(2) Others equip simulated users with large or unconstrained action spaces, making interactions difficult to control, reproduce, or evaluate reliably.
(3) Some depend on LLM-based evaluators to assess communication quality or task completion, introducing instability and compromising evaluation reliability.

To fill this gap, we introduce Interactive AppWorld, which extends AppWorld by adding the agent–user interaction dimension. 
\jane{I would personally prefer to not frame this as "Appworld++", but more like "We introduce a new benchmark using Appworld as the backbone". But I defer to Harsh's opinion.} \ashish{I see value in doing so} \harsh{+1 to Jane's framing.}
We make the following contributions:

\junzhi{re-organize it, and connect it with the gaps from the existing work}

\paragraph{1) Task Perturbation Pipeline}
We introduce a systematic pipeline \jane{"Pipeline" makes it sound like it's LLM-generated, which we claimed it wasn't a few paragraphs above} \ashish{agreed. Would it help to qualify it as ``LLM-assisted manual pipeline''?}
\harsh{The usage of LLM here is soo nominal/less, it's not even worth discussing here. It could be a footnote-level detail in the main method section. But yes, the word pipeline is better to avoid.} that perturbs existing AppWorld tasks and transforms them into scenarios that require user interaction to complete.

\paragraph{2) Diverse and Realistic Tasks}
\junzhi{emphasize the diversity of interactive tasks here}
We manually create this benchmark 
by perturbing existing Appworld tasks, resulting in 300+ interactive tasks spanning 9 everyday apps (400+ APIs) and covering three major interaction settings: unsolvable, underspecified, and confirmation-required tasks. These tasks reflect realistic user–agent dynamics while preserving AppWorld’s original complexity. 
\jane{How much do we want to push on the "realistic" angle? In my experience reviewers lock on to claims of realism to complain about use of simulated users, though opinions might have changed over the past year.} \ashish{good point. We have to keep in mind that `realistic' here should be about what's introduced, i.e., realistic agent-user interactions (not the realism of original AppWorld tasks). As long as we clearly explain/argue later that the injected interactions are realistic and common, this is OK. But agreed, need to be careful if we emphasize this.}

\paragraph{3) Highly Controllable Simulated User}
We design a carefully constrained simulated user that provides only perturbation-relevant feedback. \jane{We can't both claim that the dynamics are realistic if the user is also highly constrained. We need to address this framing so it's consistent.} This design yields a highly controllable and reliable environment for evaluating collaborative agent behaviors.

\paragraph{4) Programmatic and Robust Evaluation}
We develop a programmatic evaluation suite \jane{What is programmatic..?} \ashish{:-)  this came up often when Harsh used in the AppWorld paper. refers to using a reliable program to do evaluation, as opposed to reference matching, human eval, etc. Again, the contribution here would be about how we are doing evaluation given the newly added agent-user interaction dimension, not what we inherit because we started with AppWorld. What do we have to say in that regard?} that measures not only task correctness, but also whether an agent can appropriately communicate with the user.

\paragraph{5) Benchmarking Collaborative Agent Capabilities}
We benchmark a range of state-of-the-art LLM-based agents and reveals substantial gaps in their collaborative abilities. \ashish{as we were discussing earlier, ``collaborative'' isn't a suitable term here, as it implies the user doing some part of the task (directly in the environment) alongside the agent.}


==> _sections/method-detailed-scratch.tex <==
\section{Interactive Appworld}

\harsh{This section is outdated. Please see previous sections.}

We aim to construct a collection of natural, diverse, interaction-required, and challenging tasks that reflect a wide range of day-to-day scenarios. Given that AppWorld already provides high-quality and realistic task scenarios, 
\jane{This reads a little effusive—might be clearer to frame AppWorld as the base environment (for realism/comparability), and then state our extension/contribution explicitly} \ashish{agreed}
our strategy is to perturb existing AppWorld tasks and transform them into tasks that require user interaction. To achieve this, we modify the task generator of AppWorld, which includes Setup, Evaluation, and Solution programs as described below. The resulting tasks preserve the richness of AppWorld while adding requirements for agent–user collaboration.

\subsection{Types of Interactive Tasks}
\label{subsubsection: Types of Interactive Tasks}
To reflect how human–agent collaboration naturally unfolds in real-world settings,
\jane{Again, "realism" vs. "controllability" conflict here}
we design three major categories of interaction-required tasks: unsolvable, underspecified, and confirmation-required. These categories capture the essential modes of agent–user interaction commonly observed in practice: seeking missing information, reporting unsolvable problem, resolving ambiguity, and obtaining explicit approval for potentially risky or user-sensitive actions.

\junzhi{Add an example for each  kind of tasks in the appendix}

% \junzhi{Use a table here for different kinds of interactive tasks and their sub-categories.}

\begin{table}[t]
\centering
\small
% \setlength{\tabcolsep}{6pt}     % 列间距可微调
% \renewcommand{\arraystretch}{1.05} % 全局行距稍微加一点

\begin{tabularx}{\linewidth}{lX}
\toprule
\textbf{Task Category} & \textbf{Perturbation Type} \\
\midrule

\multirow{4}{*}{\textbf{Unsolvable}}
& Require unavailable resources \\
\addlinespace[2pt]
& Call for invalid actions\\
\addlinespace[2pt]
& Require non-existent actions\\
\addlinespace[2pt]
& Contradict common sense\\
\midrule

\multirow{2}{*}{\textbf{Vague User Intent}}
& Imply divergent end states \\
\addlinespace[2pt]
& Impose conflicting goals \\
\midrule

\multirow{3}{*}{\textbf{Confirmation-Required}}
& Confirmation required and granted \\
\addlinespace[2pt]
& Confirmation required and denied \\
\addlinespace[2pt]
& No Confirmation required \\
\bottomrule
\end{tabularx}

\caption{Category of interactive tasks. \jane{I'd add counts here, and direct the user to examples in a section of the appendix.}} \junzhi{Our categorization of interactive tasks is based on: (1)Unsolvable: User's goal can't be completed, (2)Underspecified: User's goal is vague(multiple possible end state) (3) Confirmation-Required: User's goal is clear and solvable, but confirmation is required. Underspecified isn't clear enough for our definition here. Maybe we can change it into vague/unclear user intent?}
\label{tab:interactive-taxonomy}
\end{table}



\paragraph{Unsolvable}
An unsolvable task is one where, after perturbation, no valid trajectory exists for the agent to complete the task without obtaining additional information from the user. We generate unsolvable tasks through several mechanisms: \jane{This is like the eighth numbered list listed back to back with no line breaks, we need to find a cleaner way of delivering this information lol}
\textbf{1) API Constraints:} Introducing environment states that cause API calls to fail. E.g. The agent is instructed to pay a bill via Venmo, but the account balance is insufficient.
\textbf{2) Required Items or Information Are Missing:} Removing entities or attributes from the database so that the user’s request cannot be satisfied. E.g. The user asks for a red T-shirt with rating above 4, but no such item exists in the database.
\textbf{3) Task Requires a Non-Existent Action:} Modifying the instruction to require an action for which no API can carry out. E.g. Asking the agent to “enable two-factor authentication for Venmo” when the Venmo app exposes no such API.
\textbf{4) Violations of Common-Sense or Real-World Logic:} Creating instructions that contradict basic world knowledge or temporal constraints. E.g. Asking the agent to “set a phone alarm for a time that has already passed.”

\jane{Adding on to previous comment, the formatting is too hard to read -- my eyes glaze right over it, and the paragraph headers being identical to the bullet list item titles is very difficult to parse.}
In all cases, the task becomes solvable only if the agent recognizes the impossibility and requests clarification or alternative instructions from the user.


% After perturbation, there is no possible trajectories for the agent to complete the tasks. This can be done by: 1) \textbf{API Constraints} Introducing API error in the environment. E.g. not enough money in venmo for the agent to pay the bill, 2) \textbf{Item/Information Required Doesn’t Exist} Deleting some required items/information from the database. E.g. user wants to buy a red t-shirt with ratings more than 4, but there are no such t-shirt in the database 3) \textbf{Task Requiring Non-Existent Action} Adding additional requirement in the instruction such that there is no API that can be used to complete the task. E.g. Ask the agent to turn on the two factor authentication, but there is no relevant api that can do this.  4) \textbf{Violations of Common Sense or Real-World Logic} The task given to agent contradicts basic real-world knowledge or logical consistency. E.g. set phone alarm before current time.

\paragraph{Underspecified}
An underspecified task is one where multiple trajectories appear feasible, and the agent must seek clarification to determine the user’s intended goal. Perturbations include:
\textbf{1) Multiple Valid Items Satisfy the Requirements:} Adjusting the dataset so that several candidate entities match the user’s request. E.g. The user asks the agent to send “the exercise plan note” to a workout partner, but two such notes exist.
\textbf{2) Contradictory Requirements:} Introducing conflicting or mutually exclusive constraints that prevent the agent from selecting a single correct action.
\textbf{3) Instruction-Level Underspecification:} Removing necessary details—such as item names, recipients, quantities, or conditions—so the agent cannot proceed without additional information.

These tasks solution path becomes clear only when the agent actively identifies the ambiguity and engages the user to refine the instruction.

\paragraph{Confirmation-Required Tasks}
In confirmation-required tasks, the user explicitly instructs the agent to request approval under certain conditions, typically involving cost, risk, or sensitive operations. E.g. "If the shoes you are about to purchase cost more than \$70, ask me for confirmation before buying." For each such scenario, we construct three task variants to comprehensively evaluate agent behavior:
\textbf{1) Confirmation required and the user approves:} The agent should ask for confirmation and act upon the user’s approval.
\textbf{2) Confirmation required and the user denies:} The agent must ask for confirmation and avoid executing the action when the user forbids it.
\textbf{2) Confirmation not required:} The agent should proceed without asking for confirmation, ensuring it does not over-query the user.

These variants allow us to test whether agents understand conditional confirmation logic, avoid unsafe actions, and appropriately incorporate user feedback.


% After perturbation, there are multiple trajectories for the agent to complete the tasks. The agent doesn't know which direction to choose and need user's clarification. These can be done by: 1)\textbf{Multiple items satisfied the requirements} Modifying the dataset such that there are multiple items that can meet user's requirement. E.g. user wants the agent send his workout partner an exercise plan note from his simple note, but there are two such notes. 2) \textbf{Contradictory Requirements} Task includes conflicting or mutually exclusive instructions, agent can't determine which instruction should be completed. 3) \textbf{Underspecification in the Instruction} Removing necessary information from the user instruction.

% \paragraph{Confirmation Required}
% User explicitly requires the agent to ask for confirmation under specific scenarios. E.g. user requires the agent to ask for confirmation if the price of the shoes the agent is going to buy is higher than \$70. For each scenarios, we will create confirmation tasks covering all of the three situations: 1) Confirmation is required, and the user confirm the action 2) Confirmation is required, and the user forbid the action 3) confirmation is not required, the agent should execute task without asking for any confirmation.

\subsection{Perturbation Pipeline}

% \begin{figure}[htb]
%   \vskip 0.2in
%   \begin{center}
%     \centerline{\includegraphics[width=\columnwidth]{figures/Pipeline.pdf}}
%     \caption{Perturbation Pipeline.}
%     \label{fig:pipeline}
%   \end{center}
% \end{figure}

Our task perturbation pipeline consists of three major components:
(1) LLM-guided condition extraction,
(2) Manual perturbation, and
(3) QA pair construction.

Together, these steps transform AppWorld’s originally clear and solvable task scenarios into interaction-required tasks that preserve realism while introducing agent–user collaboration.
% We first utilize an LLM to generate the conditions that makes the task clearly solvable based on the setup and solution code of the scenarios. A human expert is then making perturbations based on these conditions. For each task scenarios, we generate 3 interactive tasks for each kinds of interaction settings.
\paragraph{Step 1: LLM-Guided Condition Extraction}
We begin by analyzing each original AppWorld task to identify the necessary conditions required to make it clear and solvable. To do this, we provide an LLM with three sources of information:
1) Task instruction: the natural-language description of the user’s request
2) Task setup program: the environment initialization code
3) Solution program: the golden solution code written by human expert to solve the task.

(Note: a human-written textual explanation, originally created by AppWorld experts to document the code summary, will be used in place of the complex setup and solution code)

The LLM is asked to generate a set of conditions that guarantee the task is: 1) \textbf{Clear}: the task’s objective is unambiguous and leads to a single end state. 2) \textbf{Solvable}: the environment provides all necessary items and information, database entries are consistent with the task requirements, and all APIs invoked in the solution are executable without errors.

These extracted conditions serve as a blueprint for identifying where perturbations can be introduced without breaking realism or internal task coherence.

\paragraph{Step 2: Manual Perturbation}
Next, human experts use the extracted conditions, along with the original task generator program, to design perturbations that convert each task scenario into three distinct interactive task scenarios (as defined in §~\ref{subsubsection: Types of Interactive Tasks}).

This step involves modifying the task instruction and the initial environment state. Examples include:
\textbf{Instruction perturbation:} E.g. removing essential information, injecting ambiguities and adding new requirements.
\textbf{Dataset perturbation:} E.g. altering database entries to remove required items or introduce duplicates, injecting states that cause certain API calls to fail (e.g., setting a payment card’s balance to be insufficient), modifying user profiles or app states so that the task becomes incomplete, contradictory, or risk-sensitive.

Crucially, human experts ensure that each perturbed task aligns with real-world semantics while requiring user interaction to complete.

\paragraph{Step 3: QA Pair Construction}
After perturbing a task, we construct two sets of interaction rules that guide the simulated user:
\textbf{Allowed QA pairs:} The questions represent possible query the agent may ask in response to the injected perturbations, The answers represent the correct user feedback needed to resolve api errors, missing information, ambiguity, or confirmation requirements.
\textbf{Forbidden QA pairs:} Specific questions that the agent should not ask (e.g., requesting information the user explicitly forbids, or attempting to bypass logical constraints). The simulated user must respond to these questions with a fixed refusal template.

These QA pairs form the backbone of the interactive environment, enabling controlled and reliable agent–user communication, and laying the foundation for the simulated user.

\subsection{Simulated User}
\jane{We need to defend our choice of using a controlled, rules-based sim, and reconcile it with our earlier claims of realism.}
We implement a controlled, rules-grounded simulated user that provides only perturbation-relevant feedback while avoiding any unintended or hallucinated information. At each interaction turn, the simulated user takes the agent query and the perturbation rules as input and produces two outputs-a thinking trace and a response:
$$thinking, response = M(q, I, A, F)$$
where $q$ is the agent’s query, $I$ is the instruction of the interactive task, $A$ is the set of allowed QA pairs, $F$ is the set of forbidden QA pairs and $M$ is the Large language models used as the simulated user. The thinking output by simulated user is in the format of "\textless think\textgreater…\textless /think\textgreater", which describes whether the query matches any allowed or forbidden QA rule and why. And the response is in the format of "\textless response\textgreater…\textless /response\textgreater", which is the message returned to the agent.

\jane{pls no more numbered lists :'))))))}
Given a query $q$, 1) If $q$ matches any allowed QA pairs from $A$, the simulated user returns the corresponding predefined answer from $A$. This provides the exact missing information, clarification, or confirmation needed to resolve the perturbation. 2) If $q$ matches any forbidden QA pairs from $F$, the simulated user must output a fixed rejection response from $F$. This prevents leakage of unintended information or bypassing the intended difficulty. 3) If $q$ matches neither allowed nor forbidden QA pairs, The simulated user returns a fallback message: “Find/Decide it yourself, ask a different question, or give me more details so I can help you.” This ensures the user not to hallucinates information for the agent.

Agent queries sometimes can contain multiple sub-questions (e.g., asking about several allowed, forbidden, and irrelevant topics simultaneously in one turn). The simulated user can match the query to multiple question-answer pairs from A and F, and provide appropriate response for all of them in one turn. An example output of simulated user can be seen at Figure~\ref{fig:sim-user-format}.

\begin{figure}[htb]
  \vskip 0.2in
  \begin{center}
    \centerline{\includegraphics[width=\columnwidth]{figures/Simulated_User.pdf}}
    \caption{Example output of simulated user.}
    \label{fig:sim-user-format}
  \end{center}
\end{figure}

% \begin{figure}[t]
% \centering

% \begin{tcolorbox}[
%   title=\textbf{Agent},
%   colback=agentbg, colframe=framegray,
%   boxrule=0.6pt, arc=3pt,
%   left=6pt, right=6pt, top=6pt, bottom=6pt
% ]

% The following friends haven't replied yet: Jose Harrison, Jennifer Powell, Susan Burton, ..., Michael Burch, Connor Brown.

% \end{tcolorbox}

% \vspace{4pt}

% \begin{tcolorbox}[
%   title=\textbf{Simulated USER},
%   colback=userbg, colframe=frameblue,
%   boxrule=0.8pt, arc=3pt,
%   left=6pt, right=6pt, top=6pt, bottom=6pt
% ]
% {\ttfamily\footnotesize\textcolor{gray}{\textbf{\textless think\textgreater}}}\\
% {\itshape\footnotesize
% Based on PROHIBITED\_Q1, I should respond with "You don't have to ask for my
% confirmation for this." for people other than Michael Burch and Susan Burton;
% Based on ALLOWED\_Q1, I should response "Let me ask Michael Burch again. OK,
% Michael Burch will come." for Michael Burch; Based on ALLOWED\_Q2, I should
% response "Let me ask Susan Burton again. OK, Susan Burton will not come." for
% Susan Burton.
% }\\[-2pt]
% {\ttfamily\footnotesize\textcolor{gray}{\textbf{\textless /think\textgreater}}}

% \vspace{3pt}

% {\ttfamily\footnotesize\textcolor{black}{\textbf{\textless response\textgreater}}}\\
% {\footnotesize
% Let me ask Michael Burch again. OK, Michael Burch will come; Let me ask Susan
% Burton again. OK, Susan Burton will not come; For the other people, you don't
% have to ask for my confirmation.
% }\\[-2pt]
% {\ttfamily\footnotesize\textbf{\textless /response\textgreater}}
% \end{tcolorbox}

% \caption{Example of the simulated user’s response format.}
% \label{fig:sim-user-format}
% \end{figure}


% For each task, we will set list of allowed questions and their corresponding answers that can help agent complete the task. These response can be to specify additional requirements, confirm an action or even revert its previous instruction. During agent execution process, the simulated user is provided with original task instruction and the lists of allowed and not allowed qa pairs. When a query is asked by agent using the supersor.message\_supervisor api, the simulated user must identify which of the allowed questions the agent has asked, if agent asks an allowed question, provide the correct information according to allowed answer; when the agent asks irrelevant questions, do not provide any information.

% \subsection{Setup}
% Setup program in AppWorld is a program that instantiates tasks using three inputs: (i) Task scenario (ii) Base DB (iii) Base date and time. We will modify this generator program to generate interactive tasks.


% \subsection{Evaluation}
% \subsection{Validation}
\subsection{Final Dataset}


==> code/colorcoding_python.tex <==
\DeclareFixedFont{\ttb}{T1}{txtt}{bx}{n}{9} % for bold
\DeclareFixedFont{\ttm}{T1}{txtt}{m}{n}{9}  % for normal
\definecolor{codedeepblue}{rgb}{0,0,0.5}
\definecolor{codedeepred}{rgb}{0.6,0,0}
\definecolor{codedeepgreen}{rgb}{0,0.5,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{backcolour}{rgb}{0.95,0.95,0.95}
\lstset{ 
  backgroundcolor=\color{backcolour},  
  basicstyle=\footnotesize,        
  breakatwhitespace=false, 
  breaklines=true,              
  captionpos=b,                 
  commentstyle=\color{codedeepred}\textit,    
  frame=tb,	                   	
  keepspaces=true,                
  keywordstyle=\color{codedeepblue}\bfseries, 
  language=Python,
  otherkeywords={*,...},    
  numbers=none,  
  numbersep=5pt,              
  numberstyle=\tiny\color{commentsColor}, 
  rulecolor=\color{white},        
  showspaces=false,                
  showstringspaces=false,          
  showtabs=false,                  
  stepnumber=1,                   
  stringstyle=\color{codedeepgreen},
  tabsize=2
}

==> code/summary.tex <==
\newcommand{\listingsttfamily}{\fontfamily{IBMPlexMono-TLF}\small}
\definecolor{backcolour}{rgb}{0.95,0.95,0.95}
\lstdefinestyle{yaml}{
     basicstyle=\color{blue}\footnotesize\listingsttfamily,
     rulecolor=\color{black},
     string=[s]{'}{'},
     stringstyle=\color{blue},
     comment=[l]{:},
     commentstyle=\color{black},
     showspaces=false,                
    showstringspaces=false,          
    showtabs=false,          
     morecomment=[l]{-}
 }

\lstinputlisting[basicstyle=\ttfamily,style=yaml]{images/appendix/summary.yaml}


==> figures/simulated_user_llms.tex <==
\begin{figure}[ht]
    \centering
    \scalebox{1}{
    \includegraphics[width=1\linewidth]{images/simulate_user_llms.pdf}
    }
    \caption{Comparison of I-TGC and I-SGC of gpt-4.1 ReAct agent across different simulated users.}
    \label{fig:simulated_user_llms}
\end{figure}

==> legacy_tables.tex <==
% \begin{table*}[htb]
%   \centering
%   \small
%   \label{tab:main-results}
%   \scalebox{0.75}{
%   \begin{tabular}{l|l|ccc|ccc|ccc|ccc}
%     \toprule
%     \multirow{2}{*}{Base LLM} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Unsolvable} &  \multicolumn{3}{c}{Underspecified} & \multicolumn{3}{c}{Confirmation} & \multicolumn{3}{c}{Aggregate}\\
%     & & I-TGC & I-SGC & Recall & I-TGC & I-SGC & Recall & I-TGC & I-SGC & Recall & I-TGC & I-SGC & Recall  \\
%     \midrule
%     \multirow{2}{*}{GPT4$^{\text{O}}$}
%       & ReAct        & $11.8$ & $2.9$ & $38.2\%$ & $0.0$ & $0.0$ & $6.9\%$ & $18.6$ & $5.9$ & $58.5\%$ & $10.1$ & $0.0$ & $34.5\%$ \\
%       & FunCall    & $8.8$ & $0.0$ & $32.4\%$ & $0.0$ & $0.0$ & $1.0\%$ & $12.8$ & $5.9$ & $40.7\%$ & $7.2$ & $0.0$ & $24.7\%$ \\
%     \midrule
%     \multirow{2}{*}{GPT4.1}
%       & ReAct        & $27.5$ & $5.9$ & $61.8\%$ & $8.8$ & $0.0$ & $20.6\%$ & $31.4$ & $14.7$ & $72.3\%$ & $22.6$ & $0.0$ & $51.6\%$ \\
%       % & PlanExec     & 44.6\,|\,23.2 & 19.7\,|\,7.9 \\
%       & FunCall    & $8.8$ & $2.9$ & $34.3\%$ & $1.0$ & $0.0$ & $2.0\%$ & $16.7$ & $5.9$ & $50.7\%$ & $8.8$ & $0.0$ & $29.0\%$ \\
%     \midrule
%     \multirow{2}{*}{GPT5}
%       & ReAct        & $\underline{38.2}$ & $14.7$ & $\underline{72.5\%}$ & $\textbf{35.3}$ & $\textbf{17.6}$ & $\textbf{54.9\%}$ & $41.2$ & $20.6$ & $66.8\%$ & $\textbf{38.2}$ & $0.0$ & $\textbf{64.7\%}$ \\
%       % & PlanExec     & \textbf{32.7}\,|\,16.1 & 11.0\,|\,3.6 \\
%       & FunCall    & $21.6$ & $11.8$ & $\underline{72.5\%}$ & $\underline{23.5}$ & $5.9$ & $\underline{45.1\%}$ & $24.5$ & $14.7$ & $68.0\%$ & $23.2$ & $0.0$ & $61.9\%$ \\
%     \midrule
%     \multirow{2}{*}{Gemini3$^{\text{Pro}}$}
%       & ReAct        & $27.5$ & $14.7$ & $59.8\%$ & $22.6$ & $2.9$ & $38.2\%$ & $\underline{44.1}$ & $\underline{23.5}$ & $70.0\%$ & $31.4$ & $0.0$ & $56.0\%$ \\
%       & FunCall & $37.2$ & $\underline{20.6}$ & $67.6\%$ & $\underline{23.5}$ & $\underline{11.8}$ & $39.2\%$ & $37.2$ & $20.6$ & $66.3\%$ & $32.7$ & $0.0$ & $57.7\%$ \\
%     \midrule
%     \multirow{2}{*}{Claude$^{\text{Opus 4.5}}$}
%       & ReAct        & $\textbf{43.1}$ & $\textbf{26.5}$ & $\textbf{77.5\%}$ & $15.7$ & $2.9$ & $38.2\%$ & $\textbf{52.9}$ & $\textbf{29.4}$ & $\textbf{77.5\%}$ & $\underline{37.2}$ & $0.0$ & $\underline{64.4\%}$ \\
%       & FunCall & $18.6$ & $5.9$ & $61.8\%$ & $22.6$ & $\underline{11.8}$ & $43.1\%$ & $\underline{44.1}$ & $\textbf{29.4}$ & $\underline{76.6\%}$ & $28.4$ & $0.0$ & $60.5\%$ \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Main Results.}
% \end{table*}
% \begin{table*}[htb]
%   \centering
%   \small
%   \label{tab:main-results}
%   \scalebox{0.70}{
%   \begin{tabular}{l|l|ccc|ccc|ccc|ccc}
%     \toprule
%     \multirow{2}{*}{Base LLM} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Unsolvable} &  \multicolumn{3}{c}{Underspecified} & \multicolumn{3}{c}{Confirmation} & \multicolumn{3}{c}{Aggregate}\\
%     & & TGC & SGC & Recall & TGC & SGC & Recall & TGC & SGC & Recall & TGC & SGC & Recall  \\
%     \midrule
%     \multirow{3}{*}{GPT4$^{\text{O}}$}
%       & ReAct        & $11.8\;\textcolor{red}{\downarrow 26.4}$ & $2.9\;\textcolor{red}{\downarrow 20.6}$ & $38.2\%$ & $7.8\;\textcolor{red}{\downarrow 30.4}$ & $0.0\;\textcolor{red}{\downarrow 23.5}$ & $6.9\%$ & $23.5\;\textcolor{red}{\downarrow 14.7}$ & $5.9\;\textcolor{red}{\downarrow 17.6}$ & $58.5\%$ & $14.4\;\textcolor{red}{\downarrow 23.8}$ & $0.0\;\textcolor{red}{\downarrow 23.5}$ & $34.5\%$ \\
%       % & PlanExec     & 44.6\,|\,23.2 & 19.7\,|\,7.9 \\
%       & FullCode & $1.0\;\textcolor{red}{\downarrow 16.6}$ & $0.0\;\textcolor{red}{\downarrow 11.8}$ & $23.5\%$ & $3.9\;\textcolor{red}{\downarrow 13.7}$ & $0.0\;\textcolor{red}{\downarrow 11.8}$ & $1\%$ & $1.0\;\textcolor{red}{\downarrow 16.6}$ & $0.0\;\textcolor{red}{\downarrow 11.8}$ & $24.5\%$ & $2.0\;\textcolor{red}{\downarrow 15.6}$ & $0.0\;\textcolor{red}{\downarrow 11.8}$ & $16.4\%$ \\
%       & FunCall    & $10.8\;\textcolor{red}{\downarrow 20.6}$ & $0.0\;\textcolor{red}{\downarrow 17.6}$ & $32.4\%$ & $9.8\;\textcolor{red}{\downarrow 21.6}$ & $0.0\;\textcolor{red}{\downarrow 17.6}$ & $1.0\%$ & $18.6\;\textcolor{red}{\downarrow 12.8}$ & $5.9\;\textcolor{red}{\downarrow 11.7}$ & $40.7\%$ & $13.1\;\textcolor{red}{\downarrow 18.3}$ & $0.0\;\textcolor{red}{\downarrow 17.6}$ & $24.7\%$ \\
%     \midrule
%     \multirow{4}{*}{GPT5$^{\text{Medium}}$}
%       & ReAct        & $40.2\;\textcolor{red}{\downarrow 33.3}$ & $17.6\;\textcolor{red}{\downarrow 32.4}$ & $72.5\%$ & $46.1\;\textcolor{red}{\downarrow 27.4}$ & $20.6\;\textcolor{red}{\downarrow 29.4}$ & $54.9\%$ & $53.9\;\textcolor{red}{\downarrow 19.6}$ & $29.4\;\textcolor{red}{\downarrow 20.6}$ & $66.8\%$ & $46.7\;\textcolor{red}{\downarrow 26.8}$ & $2.9\;\textcolor{red}{\downarrow 47.1}$ & $64.7\%$ \\
%       % & PlanExec     & \textbf{32.7}\,|\,16.1 & 11.0\,|\,3.6 \\
%       & FullCode & $1.0\;\textcolor{red}{\downarrow 19.6}$ & $0.0\;\textcolor{red}{\downarrow 5.9}$ & $21.6\%$ & $6.9\;\textcolor{red}{\downarrow 13.7}$ & $0.0\;\textcolor{red}{\downarrow 5.9}$ & $12.7\%$ & $2.0\;\textcolor{red}{\downarrow 18.6}$ & $0.0\;\textcolor{red}{\downarrow 5.9}$ & $26.5\%$ & $3.3\;\textcolor{red}{\downarrow 17.3}$ & $0.0\;\textcolor{red}{\downarrow 5.9}$ & $20.3\%$ \\
%       & FunCall    & $23.5\;\textcolor{red}{\downarrow 23.6}$ & $11.8\;\textcolor{red}{\downarrow 23.5}$ & $72.5\%$ & $29.4\;\textcolor{red}{\downarrow 17.7}$ & $5.9\;\textcolor{red}{\downarrow 29.4}$ & $45.1\%$ & $33.3\;\textcolor{red}{\downarrow 13.8}$ & $20.6\;\textcolor{red}{\downarrow 14.7}$ & $68.0\%$ & $28.8\;\textcolor{red}{\downarrow 18.3}$ & $0.0\;\textcolor{red}{\downarrow 35.3}$ & $61.9\%$ \\
%     \midrule
%     \multirow{3}{*}{Gemini}
%       & ReAct        & - & - & - & - & - & - & - & - & - & - & - & - \\
%       & FullCode     & - & - & - & - & - & - & - & - & - & - & - & - \\
%       & FunCall & - & - & - & - & - & - & - & - & - & - & - & - \\
%     \midrule
%     \multirow{3}{*}{Claude}
%       & ReAct        & - & - & - & - & - & - & - & - & - & - & - & - \\
%       & FullCode     & - & - & - & - & - & - & - & - & - & - & - & - \\
%       & FunCall & - & - & - & - & - & - & - & - & - & - & - & - \\
%     \midrule
%     \multirow{3}{*}{LLaMA3}
%       & ReAct        & - & - & - & - & - & - & - & - & - & - & - & - \\
%       % & PlanExec     & 8.9\,|\,1.8  & 2.4\,|\,0.7 \\
%       & FullCode & - & - & - & - & - & - & - & - & - & - & - & - \\
%     \midrule
%     \multirow{3}{*}{DeepSeek}
%       & ReAct        & - & - & - & - & - & - & - & - & - & - & - & - \\
%       % & PlanExec     & 1.8\,|\,0.0 & 0.7\,|\,0.0 \\
%       & FullCode & - & - & - & - & - & - & - & - & - & - & - & - \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Main Results. $\textcolor{red}{\downarrow number}$ indicates the amount of performance degradation relative to the original setting.}
% \end{table*}

% \begin{table*}[htb]
%   \centering
%   \small
%   \label{tab:main-results}
%   \scalebox{0.90}{
%   \begin{tabular}{l|l|cc|cc|cc|cc}
%     \toprule
%     \multirow{2}{*}{Base LLM} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{Unsolvable} &  \multicolumn{2}{c}{Underspecified} & \multicolumn{2}{c}{Confirmation} & \multicolumn{2}{c}{Aggregate}\\
%     & & TGC & Recall & TGC & Recall & TGC & Recall & TGC & Recall  \\
%     \midrule
%     \multirow{2}{*}{GPT4$^{\text{O}}$}
%       & ReAct        & $11.8\;\textcolor{red}{\downarrow 26.4}$ & $38.2\%$ & $7.8\;\textcolor{red}{\downarrow 30.4}$ & $6.9\%$ & $23.5\;\textcolor{red}{\downarrow 14.7}$ & $58.5\%$ & $14.4\;\textcolor{red}{\downarrow 23.8}$ & $34.5\%$ \\
%       & FunCall    & $10.8\;\textcolor{red}{\downarrow 20.6}$ & $32.4\%$ & $9.8\;\textcolor{red}{\downarrow 21.6}$ & $1.0\%$ & $18.6\;\textcolor{red}{\downarrow 12.8}$ & $40.7\%$ & $13.1\;\textcolor{red}{\downarrow 18.3}$ & $24.7\%$ \\
%     \midrule
%     \multirow{2}{*}{GPT4.1}
%       & ReAct        & $27.5\;\textcolor{red}{\downarrow 22.5}$ & $61.8\%$ & $26.5\;\textcolor{red}{\downarrow 23.5}$ & $20.6\%$ & $40.2\;\textcolor{red}{\downarrow 9.8}$ & $72.3\%$ & $31.4\;\textcolor{red}{\downarrow 18.6}$ & $51.6\%$ \\
%       % & PlanExec     & 44.6\,|\,23.2 & 19.7\,|\,7.9 \\
%       & FunCall    & $13.7\;\textcolor{red}{\downarrow 20.6}$ & $34.3\%$ & $16.7\;\textcolor{red}{\downarrow 17.6}$ & $2.0\%$ & $26.5\;\textcolor{red}{\downarrow 7.8}$ & $50.7\%$ & $18.9\;\textcolor{red}{\downarrow 15.4}$ & $29.0\%$ \\
%     \midrule
%     \multirow{2}{*}{GPT5$^{\text{Medium}}$}
%       & ReAct        & $40.2\;\textcolor{red}{\downarrow 33.3}$ & $72.5\%$ & $46.1\;\textcolor{red}{\downarrow 27.4}$ & $54.9\%$ & $53.9\;\textcolor{red}{\downarrow 19.6}$ & $66.8\%$ & $46.7\;\textcolor{red}{\downarrow 26.8}$ & $64.7\%$ \\
%       % & PlanExec     & \textbf{32.7}\,|\,16.1 & 11.0\,|\,3.6 \\
%       & FunCall    & $23.5\;\textcolor{red}{\downarrow 23.6}$ & $72.5\%$ & $29.4\;\textcolor{red}{\downarrow 17.7}$ & $45.1\%$ & $33.3\;\textcolor{red}{\downarrow 13.8}$ & $68.0\%$ & $28.8\;\textcolor{red}{\downarrow 18.3}$ & $61.9\%$ \\
%     \midrule
%     \multirow{2}{*}{Gemini}
%       & ReAct        & - & - & - & - & - & - & - & - \\
%       & FunCall & - & - & - & - & - & - & - & - \\
%     \midrule
%     \multirow{2}{*}{Claude}
%       & ReAct        & - & - & - & - & - & - & - & - \\
%       & FunCall & - & - & - & - & - & - & - & - \\
%     \midrule
%     \multirow{2}{*}{xAI}
%       & ReAct        & - & - & - & - & - & - & - & - \\
%       & FunCall & - & - & - & - & - & - & - & - \\
%     \midrule
%     \multirow{1}{*}{Kimi-K2}
%       & ReAct        & - & - & - & - & - & - & - & - \\
%     \midrule
%     \multirow{1}{*}{Qwen}
%       & ReAct        & - & - & - & - & - & - & - & - \\
%     \midrule
%     \multirow{1}{*}{DeepSeek}
%       & ReAct        & - & - & - & - & - & - & - & - \\
%       % & PlanExec     & 1.8\,|\,0.0 & 0.7\,|\,0.0 \\
%       % & FullCode & - & - & - & - & - & - & - & - & - & - & - & - \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Main Results. $\textcolor{red}{\downarrow number}$ indicates the amount of performance degradation relative to the original setting.}
% \end{table*}

% \begin{table*}[htb]
%   \centering
%   \small
%   \label{tab:main-results}
%   \scalebox{0.75}{
%   \begin{tabular}{l|l|ccc|ccc|ccc|cccc}
%     \toprule
%     \multirow{2}{*}{Base LLM} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Unsolvable} &  \multicolumn{3}{c}{Underspecified} & \multicolumn{3}{c}{Confirmation} & \multicolumn{4}{c}{Aggregate}\\
%     & & I-TGC & I-SGC & Recall & I-TGC & I-SGC & Recall & I-TGC & I-SGC & Recall & O-TGC & I-TGC & I-SGC & Recall  \\
%     \midrule
%     \multirow{2}{*}{GPT4$^{\text{O}}$}
%       & ReAct        & $11.8$ & $2.9$ & $38.2\%$ & $0.0$ & $0.0$ & $6.9\%$ & $18.6$ & $5.9$ & $58.5\%$ & $38.2$ & $10.1$ & $0.0$ & $34.5\%$ \\
%       & FunCall    & $8.8$ & $0.0$ & $32.4\%$ & $0.0$ & $0.0$ & $1.0\%$ & $12.8$ & $5.9$ & $40.7\%$ & $31.4$ & $7.2$ & $0.0$ & $24.7\%$ \\
%     \midrule
%     \multirow{2}{*}{GPT4.1}
%       & ReAct        & $27.5$ & $5.9$ & $61.8\%$ & $8.8$ & $0.0$ & $20.6\%$ & $31.4$ & $14.7$ & $72.3\%$ & $50.0$ & $22.6$ & $0.0$ & $51.6\%$ \\
%       % & PlanExec     & 44.6\,|\,23.2 & 19.7\,|\,7.9 \\
%       & FunCall    & $8.8$ & $2.9$ & $34.3\%$ & $1.0$ & $0.0$ & $2.0\%$ & $16.7$ & $5.9$ & $50.7\%$ & $34.3$ & $8.8$ & $0.0$ & $29.0\%$ \\
%     \midrule
%     \multirow{2}{*}{GPT5}
%       & ReAct        & $\underline{38.2}$ & $14.7$ & $\underline{72.5\%}$ & $\textbf{35.3}$ & $\textbf{17.6}$ & $\textbf{54.9\%}$ & $41.2$ & $20.6$ & $66.8\%$ & $73.5$ & $\textbf{38.2}$ & $0.0$ & $\textbf{64.7\%}$ \\
%       % & PlanExec     & \textbf{32.7}\,|\,16.1 & 11.0\,|\,3.6 \\
%       & FunCall    & $21.6$ & $11.8$ & $\underline{72.5\%}$ & $\underline{23.5}$ & $5.9$ & $\underline{45.1\%}$ & $24.5$ & $14.7$ & $68.0\%$ & $47.1$ & $23.2$ & $0.0$ & $61.9\%$ \\
%     \midrule
%     \multirow{2}{*}{Gemini3$^{\text{Pro}}$}
%       & ReAct        & $27.5$ & $14.7$ & $59.8\%$ & $22.6$ & $2.9$ & $38.2\%$ & $\underline{44.1}$ & $\underline{23.5}$ & $70.0\%$ & - & $31.4$ & $0.0$ & $56.0\%$ \\
%       & FunCall & $37.2$ & $\underline{20.6}$ & $67.6\%$ & $\underline{23.5}$ & $\underline{11.8}$ & $39.2\%$ & $37.2$ & $20.6$ & $66.3\%$ & - & $32.7$ & $0.0$ & $57.7\%$ \\
%     \midrule
%     \multirow{2}{*}{Claude$^{\text{Opus 4.5}}$}
%       & ReAct        & $\textbf{43.1}$ & $\textbf{26.5}$ & $\textbf{77.5\%}$ & $15.7$ & $2.9$ & $38.2\%$ & $\textbf{52.9}$ & $\textbf{29.4}$ & $\textbf{77.5\%}$ & - & $\underline{37.2}$ & $0.0$ & $\underline{64.4\%}$ \\
%       & FunCall & $18.6$ & $5.9$ & $61.8\%$ & $22.6$ & $\underline{11.8}$ & $43.1\%$ & $\underline{44.1}$ & $\textbf{29.4}$ & $\underline{76.6\%}$ & - & $28.4$ & $0.0$ & $60.5\%$ \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Main Results.}
% \end{table*}

% \begin{table*}[htb]
%   \centering
%   \small
%   \label{tab:main-results}
%   \scalebox{0.67}{
%   \begin{tabular}{l|l|cccc|cccc|cccc|cccc}
%     \toprule
%     \multirow{2}{*}{Base LLM} & \multirow{2}{*}{Method} & \multicolumn{4}{c}{Unsolvable} &  \multicolumn{4}{c}{Underspecified} & \multicolumn{4}{c}{Confirmation} & \multicolumn{4}{c}{Aggregate}\\
%     & & A-TGC & I-TGC & I-SGC & Recall & A-TGC & I-TGC & I-SGC & Recall & A-TGC & I-TGC & I-SGC & Recall & A-TGC & I-TGC & I-SGC & Recall  \\
%     \midrule
%     \multirow{2}{*}{GPT4$^{\text{O}}$}
%       & ReAct        & $11.8$ & $11.8$ & $2.9$ & $38.2\%$ & $7.8$ & $0.0$ & $0.0$ & $6.9\%$ & $23.5$ & $18.6$ & $5.9$ & $58.5\%$ & $14.4$ & $10.1$ & $0.0$ & $34.5\%$ \\
%       & FunCall    & $10.8$ & $8.8$ & $0.0$ & $32.4\%$ & $9.8$ & $0.0$ & $0.0$ & $1.0\%$ & $18.6$ & $12.8$ & $5.9$ & $40.7\%$ & $13.1$ & $7.2$ & $0.0$ & $24.7\%$ \\
%     \midrule
%     \multirow{2}{*}{GPT4.1}
%       & ReAct        & $27.5$ & $27.5$ & $5.9$ & $61.8\%$ & $26.5$ & $8.8$ & $0.0$ & $20.6\%$ & $40.2$ & $31.4$ & $14.7$ & $72.3\%$ & $31.4$ & $22.6$ & $0.0$ & $51.6\%$ \\
%       % & PlanExec     & 44.6\,|\,23.2 & 19.7\,|\,7.9 \\
%       & FunCall    & 13.7 & $8.8$ & $2.9$ & $34.3\%$ & $16.7$ & $1.0$ & $0.0$ & $2.0\%$ & $26.5$ & $16.7$ & $5.9$ & $50.7\%$ & $18.9$ & $8.8$ & $0.0$ & $29.0\%$ \\
%     \midrule
%     \multirow{2}{*}{GPT5}
%       & ReAct        & $40.2$ & $\underline{38.2}$ & $14.7$ & $\underline{72.5\%}$ & $\textbf{46.1}$ & $\textbf{35.3}$ & $\textbf{17.6}$ & $\textbf{54.9\%}$ & $53.9$ & $41.2$ & $20.6$ & $66.8\%$ & $\textbf{46.7}$ & $\textbf{38.2}$ & $0.0$ & $\textbf{64.7\%}$ \\
%       % & PlanExec     & \textbf{32.7}\,|\,16.1 & 11.0\,|\,3.6 \\
%       & FunCall    & $23.5$ & $21.6$ & $11.8$ & $\underline{72.5\%}$ & $29.4$ & $\underline{23.5}$ & $5.9$ & $\underline{45.1\%}$ & $33.3$ & $24.5$ & $14.7$ & $68.0\%$ & $28.8$ & $23.2$ & $0.0$ & $61.9\%$ \\
%     \midrule
%     \multirow{2}{*}{Gemini3$^{\text{Pro}}$}
%       & ReAct        & $32.4$ & $27.5$ & $14.7$ & $59.8\%$ & $\underline{35.3}$ & $22.6$ & $2.9$ & $38.2\%$ & $\underline{57.8}$ & $\underline{44.1}$ & $\underline{23.5}$ & $70.0\%$ & $41.8$ & $31.4$ & $0.0$ & $56.0\%$ \\
%       & FunCall & \underline{$42.2$} & $37.2$ & $\underline{20.6}$ & $67.6\%$ & $\underline{35.3}$ & $\underline{23.5}$ & $\underline{11.8}$ & $39.2\%$ & $51.0$ & $37.2$ & $20.6$ & $66.3\%$ & $42.8$ & $32.7$ & $0.0$ & $57.7\%$ \\
%     \midrule
%     \multirow{2}{*}{Claude$^{\text{Opus 4.5}}$}
%       & ReAct        & $\textbf{44.1}$ & $\textbf{43.1}$ & $\textbf{26.5}$ & $\textbf{77.5\%}$ & $28.4$ & $15.7$ & $2.9$ & $38.2\%$ & $\textbf{65.7}$ & $\textbf{52.9}$ & $\textbf{29.4}$ & $\textbf{77.5\%}$ & $\underline{46.1}$ & $\underline{37.2}$ & $0.0$ & $\underline{64.4\%}$ \\
%       & FunCall & $21.6$ & $18.6$ & $5.9$ & $61.8\%$ & $29.4$ & $22.6$ & $\underline{11.8}$ & $43.1\%$ & $55.9$ & $\underline{44.1}$ & $\textbf{29.4}$ & $\underline{76.6\%}$ & $35.6$ & $28.4$ & $0.0$ & $60.5\%$ \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Main Results.}
% \end{table*}

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\scalebox{0.68}{
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{Allow Interaction} & \multicolumn{2}{c}{Forbid Interaction} & \multicolumn{2}{c}{Drop} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Split & I-TGC$\uparrow$ & I-SGC$\uparrow$ & I-TGC$\uparrow$ & I-SGC$\uparrow$ & $\Delta$I-TGC & $\Delta$I-SGC \\
\midrule
All (Aggregate)      & 38.2 &  2.9 & 15.4 & 0.0 & $\textcolor{red}{-67.0\%}$ & $\textcolor{red}{-100.0\%}$ \\
Unsolvable           & 38.2 & 17.6 &  7.8 & 2.9 & $\textcolor{red}{-80.6\%}$ & $\textcolor{red}{-83.5\%}$ \\
Underspecified       & 35.3 & 20.6 & 18.6 & 0.0 & $\textcolor{red}{-59.7\%}$ & $\textcolor{red}{-100.0\%}$ \\
Confirmation         & 41.2 & 29.4 & 19.6 & 5.9 & $\textcolor{red}{-63.6\%}$ & $\textcolor{red}{-79.9\%}$ \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Interaction ablation for GPT5-Medium.} Disallowing agent-user interaction causes large drops in both task-goal completion (TGC) and scenario-goal completion (SGC), indicating that the benchmark is strongly interaction-dependent.}
\label{tab:interaction_ablation_tgc_sgc}
\end{table}

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\scalebox{0.9}{
\begin{tabular}{l|c|cc|cc}
\toprule
\multirow{2}{*}{Setting} 
& \multirow{2}{*}{O-TGC}
& \multicolumn{2}{c|}{I-TGC} 
& \multicolumn{2}{c}{I-SGC} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
&  & w/o & w & w/o & w \\
\midrule
Aggregate
& 73.5
& 38.2 & 63.1
& 0.0 & 17.6 \\

Unsolvable
& 73.5
& 38.2 & 67.7
& 14.7 & 50.0 \\

Underspecified
& 73.5
& 35.3 & 63.7
& 17.6 & 41.2 \\

Confirmation
& 73.5
& 41.2 & 57.8
& 20.6 & 26.5 \\
\bottomrule
\end{tabular}
}
\caption{
w and w/o Gold Interaction
}
\label{tab:gold_interaction_comparison}
\end{table}

==> tables/simulated_user_llms_full.tex <==
\begin{table}[htb]
\centering
\caption{
Comparison of Task Goal Completion (TGC, \%) and Interaction Recall (\%) of gpt-4.1 ReAct agent across different simulated users. \ashish{drop recall; add GPT-5; ideally add an open model too (but after submission); mark GPT-4o as default that we use}
}
\label{tab:sim_user_comparison}
\small
\setlength{\tabcolsep}{6pt}
\scalebox{0.8}{
\begin{tabular}{l|cc|cc|cc}
\toprule
\multirow{2}{*}{Setting} 
& \multicolumn{2}{c|}{GPT-4o User} 
& \multicolumn{2}{c}{GPT-4.1 User}
& \multicolumn{2}{c}{GPT-5 User}\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& I-TGC & I-SGC & I-TGC & I-SGC & I-TGC & I-SGC \\
\midrule
Aggregate
& 22.6 & 6.9
& 21.9 & 9.8
& 22.2 & 10.8 \\

Unsolvable
& 27.5 & 5.9
& 25.5 & 8.8
& 32.4 & 14.7 \\

Underspecific
& 8.8 & 0.0
& 6.9 & 2.9
& 6.9 & 2.9 \\

Confirmation
& 31.4 & 14.7
& 33.3 & 17.6
& 27.5 & 14.7 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/simulated_user_manual_evaluation.tex <==
\begin{table}[htb]
    \centering
    \caption{Manual evaluation of response from gpt-4o simulated user in the experiment of gpt-4.1 react agent}
    \label{tab:simulated_user_evaluation}
    \small
    \scalebox{0.8}{
        \begin{tabular}{ccc}
        \toprule
        fail to identify correct question &  falsely reveal information & Failure Rate\\
        \midrule
        4 & 1 & $1.6\%$ \\
        \bottomrule
        \end{tabular}
    }
\end{table}
